IEEE 802.11az Indoor Positioning with mmWave

Last years we have witnessed the uprising of location based applications, which depend on the devices ability to accurately obtain their position. IEEE 802.11, foretelling the need for such applications, started the IEEE 802.11az work on Next Generation Positioning. Although this standard provides positioning enhancements for sub-6GHz and mmWave bands, high accuracy in the order of centimeters can only be obtained in the latter band, thanks to the beamforming information available at mmWave operation. This work presents a detailed analysis on the new techniques provided by IEEE 802.11az for enhanced secured positioning in the mmWave band, assessing them through experimentation.

==> 01_introduction.tex <==
\section{Introduction}
%intro where we specify use cases that need cm-level precison from wi fi networks
With the advance of new services such as asset tracking, factory automation, autonomous robots, and logistics and distribution management; ultra-precise localization and positioning are demanded from local and personal wireless technologies~\cite{m1}. While the current sub-6~Ghz WLANs can achieve a positioning accuracy of tens of meters to tens of centimeters~\cite{m1}, the 60~Ghz WLAN with its high temporal resolution from the multi-GHz bandwidth can achieve this ultra-precise positioning accuracy. 

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{img/relative-positioning.pdf}
    \caption{Legacy positioning in 802.11
    only knew the distance between devices,
    thus, there are many feasible locations
    (blue markers). 
    802.11az uses \gls{mmwave}
    beamforming to obtain the azimuth and
    elevation between devices, hence, 
    the exact location (red marker).}
    \label{fig:relative-positioning}
\end{figure}

In the realization of this cm-level accuracy, the next-generation WLANs in the 60~Ghz band face three main challenges. First, they need to support an estimation of the distance, azimuth, and elevation between two Wi-Fi devices, which is needed for positioning (see Fig~\ref{fig:relative-positioning}). Second, knowing that the positioning performance in mmWave networks degrades when the connectivity between the two Wi-Fi devices is not directional~\cite{alejandro}, a \gls{los} assessment support is needed. Third, in order to preserve user privacy, the position estimations need to be exchanged between the Wi-Fi devices securely. 

The IEEE 802.11az amendment~\cite{802.11az} addresses these challenges, bringing new physical (PHY) and media access control (MAC) layer improvements to enable secure and accurate positioning for operation in the 60~Ghz band. These new improvements include high-precision angle and \gls{tof} estimations that are exchanged between \gls{sta}s using the Fine Timing Measurement (FTM) procedure~\cite{802.11mc}. \gls{sta}s use the exchanged estimations to determine the distance, azimuth, and elevation between \gls{sta}s -- see~Fig.~\ref{fig:relative-positioning}. Furthermore, to prevent malicious \gls{sta}s to derive users’ position from the insecure \gls{ftm} exchange, 802.11az proposes a \gls{pasn} procedure to encrypt the \gls{ftm} sessions.  

\bigskip

In recent years, various works have analyzed the security~\cite{m2,security-tof-ranging}; performance and scalability~\cite{m3} features of 802.11az for operations in the sub-6~Ghz band~\cite{az-sub6-finger}. However, non of the existing works in the literature discusses the  802.11az improvements for operation in the 60~Ghz band that promises position accuracy with 10 times bigger resolution~\cite{m5}. This article overviews those new improvements and describes the potential benefits and challenges of each one. We have grouped these improvements into three categories: \gls{ftm} protocol over \gls{edmg},~\gls{los} assessment over the first path, and secure next-generation positioning. Moreover, we also perform an experimental analysis that shows the potential positioning accuracy of future \gls{mmwave}-based implementation of 802.11az. This is followed by a discussion of several key system-level challenges for the realization of the next-generation WLAN positioning systems 


% SoA categories
{\color{red}
\begin{itemize}
    \item CSI+mmWave: \cite{alejandro,passive-mmwave,mm-track}
    \item security: \cite{m2,security-tof-ranging}
    \item 802.11az: \cite{m3} studies the latency/positioning
        tradeoff using az with communication 20~MHz and
        multi-user positioning (no angle info.).
        \cite{az-sub6-finger} uses 5~GHz SISO with 
        channel impulse response (CIR) and AI/ML fingerprinting
        (no angle information).
    \item angles+TOF~\cite{mdtrack}
    \item Bluetooth, UWB and multiple
        technologies like WiFi for hybrid
        localization~\cite{hybrid-localization}.
        \cite{uwb-denoising}~to have LOS/NLOS
        detection using denoising of CIR
        and classification
\end{itemize}
}


\todo[inline]{Jorge: why not Bluetooth, AWB
or RFID. Use the 15 refs to go on 802.11az
literature.}

\todo[inline]{Jorge: Mention other things that
az introduces, although we do not cover it.
Try to leave cristal clear that it's not a
tutorial.}

\todo[inline]{Milan: for the first challenge,
what is required is to \emph{exchange} angle,
distance info. inside the protocol exchange
(FTM).} 

\todo[inline]{Jorge/Milan: try to mention
existing location techniques: fingerprinting,
CSI estimations, AI/ML (cite Xavi's work).
Use ANOTHER ref for AZ}


\todo[inline]{Reviewer 1: The structure of the introduction is quite poor, and lacks several important aspects such as a description of (i) the contributions of the paper; (ii) the adopted methodology; (iii) the outcomes and results of the paper; (iv) the related works, and how (and whether) the paper overcomes literature’s limitations.}

\todo[inline]{Reviewer 1: Highly important aspects such as multi-user positioning, secure preamble (LTF), and passive positioning should be highlighted.}



%\gls{mmwave} WLAN positioning differs significantly from other existing positioning technologies such as visible light positioning (VLP), radio frequency identification (RFID), Bluetooth, and ultrawide-bands (UWB). In particular, WLAN positioning can provide a better transmission range while reusing the existing Wi-Fi devices which leads to a significant decrease in deployment complexity and cost.  

%https://ieeexplore.ieee.org/abstract/document/9569340 - ranging and location attacks
%Multi-User Position Estimation and PerformanceTrade-offs in IEEE 802.11az WLANs
%https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8436404 - IoT that mentoines az
%https://www.mdpi.com/2079-9292/9/8/1193

%In particular, visible light positioning (VLP) relies on detecting the visible lights emitted by LED transmitters at known locations to determine the positions of light sensors. While implementation of VLP requires specialized equipment like photodetectors and imaging sensors, which can increase the overall cost of the system [REF], the \gls{mmwave} positioning can reuse existing Wi-Fi devices that are originally deployed for communication.  

%This amendment also offers enhancements for wireless medium utilization, power consumption, and scalable dense deployments that are not in the scope of this article. This article overviews the positioning and security features related to the mmWave WLANs that have the potential to achieve the ultra-precise positioning required by the diverse services and applications that will emerge [REF]

%In addition to the 60 GHz communication, the IEEE 802.11az amendment offers positioning enhancements for the sub-6 GHz bands. However, this lower bands can no 


%To address those challenges, the IEEE 802.11az Task Group (802.11az for short) worked from 2015 to 2022 on an amendment~\cite{802.11az} that defines PHY and MAC layer enhancements to improve the WLAN positioning. Among other enhancements  

%The IEEE 802.11az amendment~\cite{802.11az} addresses these challenges, 

%To meet these demands, 

%az Task Group (802.11az for short) worked since 2015 to 2022 on an amendment~\cite{802.11az} that defines PHY and MAC updates for Next Generation Positioning.



%-how az addresses this challenges enumerate az new features, state that there are other enahncments for bla bla i bla but we foucs on the improved positioning accuracy
%Among other features, that to address the cm-level positioning needs the IEEE 802.11 az amadmand proposed modificaitons ant PHY and MAC layer for mmWave ... This is the scope of our paper, however the az amadmant also offers alternatives in sub6 GHz with multi user localization but this alternative can not achive the cm-level acuracy. 

%related work and what is currently missing
%Bluetooth and other alternatives for SoA and why not them... and also write the little soa that existn on az and basiclly that id does not cover the Indoor postioning in mmwave. What is the gap that we fill in in the literacure

%the contribution of this paper are:

%Although 802.11az provides enhancements for sub-6~GHz and \gls{mmwave} operation at 60~GHz, the best positioning accuracy is achieved in the latter band. Specifically, 802.11az obtains accurate positioning information using 802.11ay \gls{edmg} beamforming \cite{802.11ay}, along with its accurate \gls{csi} reports. With the orientation of the \gls{mmwave} beam and \gls{csi} reports, 802.11az elaborates angle estimations funded on the ranging accuracy of \mbox{multi-GHz} bandwidths.   


%Unlike \gls{rssi} based solutions~\cite{localization-survey}, 802.11az combines \gls{mmwave}-based angle estimations with  the \gls{tof} to achieve high accuracy positioning. Both the \gls{tof} and angle estimations are exchanged using the \gls{ftm} procedure -- introduced in 802.11mc~\cite{802.11mc} --, and \gls{sta}s use the exchanged estimations to determine the distance, azimuth and elevation between \gls{sta}s -- see~Fig.~\ref{fig:relative-positioning}.

%Since \gls{mmwave} promises to increase positioning accuracy from meter level~\cite{MultipathTD} to centimeter-level~\cite{mmwave-survey,joan}; in this article we explain the main contributions of 802.11az for \gls{mmwave} based positioning:



%\textbf{FTM procedure over EDMG.} In the legacy \gls{ftm} procedure \gls{sta}s only exchange \gls{tof} estimations, thus, obtaining just an approximation of the distance. 802.11az performs the \gls{ftm} procedure over \gls{edmg} to also exchange angle estimations obtained through \gls{csi} reports. Namely, \gls{sta}s exchange  the angle at which the signals depart and arrive to the \gls{sta}, i.e., the \gls{aod} and \gls{aoa}. With the distance and angle estimations it is possible to obtain the exact position of a \gls{sta} -- see Fig.~\ref{fig:relative-positioning}.\footnote{Note that throughout the paper we use blue color for legacy features, purple color for legacy features that were extended in the IEEE 802.11az amendment and red color for new features.}

% Beamforming, FPBT & LOS assessment
%\textbf{LOS assessment over the first path.} When \gls{sta}s are not at \gls{los} it becomes challenging to obtain the position due to signal reflections, e.g., on walls. Thus, it is important to determine if \gls{sta}s are at \gls{los} to derive accurate position estimations. 802.11az introduces a \gls{los} assessment procedure that tells if \gls{sta}s are at \gls{los} using dual polarization over first path transmissions. In case the \gls{los} assessment succeeds it is possible to obtain the exact position of a \gls{sta} as depicted in Fig.~\ref{fig:relative-positioning}. Otherwise, signal reflections should be considered.

% Security
%\textbf{Secure Next Generation Positioning.} Since \gls{ftm} exchanges may be triggered without association, malicious \gls{sta}s may derive users' position. To prevent that, 802.11az proposes a \gls{pasn} to exchange a key used to secure \gls{ftm} sessions between not associated \gls{sta}s. Moreover, 802.11az increases the location privacy with physical security randomizing the \gls{trn} subfields used in \gls{edmg} \gls{ppdu}s. Hence, no third party can derive estimations about other \gls{sta}s location.

%\bigskip
%The remainder of this article is as follows. Sec.~\ref{sec:ftm}-\ref{sec:secure} detail the main contributions of 802.11az \gls{mmwave}-based positioning. Next, Sec.~\ref{sec:experimental} assesses the accuracy of future 802.11az \gls{mmwave}-based implementations. Finally, Sec.~\ref{sec:challenges} identifies the existing challenges to be addressed while implementing \gls{mmwave}-based 802.11az.

%



%---DO NOT INTRODUCE DIFFICULT CONCEPTS HERE, DO NOT MENTION THEM, DO NOT SUMMARY THE PAPER, USE THE INTRODUCTION STRUCTURE UP---

%refer fig1 once 1st time elev azi

%https://www.wi-fi.org/beacon/the-beacon/wi-fi-certified-location-capabilities-demonstrated-at-lisbon-member-event
%this page antonio shared it, just to say there is work in progress on real implementations


%USE CASES OF ULTRA PRECISE POSITIONG
%1st paragraph : remove UWB and current sub6 (all soa from 1st paragraph)
%With the advance of new services such as asset tracking, factory automation, autonomous robots, and logistics and distribution management; ultra-precise localization and positioning are demanded from local and personal wireless technologies [REF]. While the current sub-6 GHz WLANs can achieve a positioning accuracy of tens of meters to tens of centimeters [REF], the 60 GHz WLAN with its high temporal resolution from the multi-GHz bandwidth can achieve this ultra-precise positioning accuracy. 

%mmwave positioinign and how is it done today

% what are the challenges /  problems of mmwave positiing today and why the mmwave postioting today can lead to high error. put here that aoa does not always travel over ftm

%how does az solve this challenge

%SoA on az !




==> 01_introduction_reviewed.tex <==
\section{Introduction}
%intro where we specify use cases that need cm-level precison from wi fi networks
With the advance of new services such as asset tracking, factory automation, autonomous robots, and logistics and distribution management; ultra-precise localization and positioning are demanded from local and personal wireless technologies~\cite{m5}. Current sub-6~GHz technologies such as 802.11, Bluetooth, and \gls{uwb} already achieve decimeter positioning accuracy~\cite{uwb-denoising,hybrid-localization}. However, ultra-precise positioning is achievable with precise position estimations at higher channel bandwidths.




\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{img/relative-positioning.pdf}
    \caption{Legacy positioning in 802.11
    only knew the distance between devices,
    thus, there are many feasible locations
    (blue markers). 
    802.11az uses \gls{mmwave}
    beamforming to obtain the azimuth and
    elevation between devices, hence, 
    the exact location (red marker).}
    \label{fig:relative-positioning}
\end{figure}




% mmWave @60GHz, precise (mention SoA)
Given the adoption of mmWave in
802.11ad/ay standards, the networking community
has studied the positioning precision at
60~GHz channels. 
Works as~\cite{alejandro,mm-track,mdtrack,passive-mmwave}
show that mmWave beamforming and
channel information helps achieving
centimeter level accuracy. Specifically,
the literature exploits the 60~GHz bandwidth of mmWave for
accurate distance, azimuth and elevation estimations -- see\footnote{Note that throughout the paper we use blue color for legacy features, purple color for legacy features that were extended in the IEEE 802.11az amendment and red color for new features.}~Fig.~\ref{fig:relative-positioning}.


% az standarizes mmWave positioning
The new IEEE~802.11az amendment~\cite{802.11az}
standardizes the positioning procedure in
mmWave. In particular, 802.11az defines
% ($i$)
the exchange of angle and \gls{tof}
information,
% ($ii$)
the beamforming procedure,
% ($iii$)
a \gls{los} assessment, and
% ($iv$)
private positioning exchanges. 
Additionally, 802.11az defines
sub-6~GHz multi-user positioning, passive
positioning and a secure preamble
mechanism.

% SoA on 802.11az
Recent works have studied diverse aspects
covered in the recent 802.11az amendment.
\cite{m3}~studies the
impact of 802.11az sub-6~GHz multi-user
positioning to the
channel delay and throughput.
\cite{az-sub6-finger}~proposes a deep learning
solution for 802.11az positioning in
sub-6~GHz channels.
While works as~\cite{m2} show that
malicious sub-6GHz
\gls{sta}s may inject wrong position
reports, or attack at a physical
level the multi-carrier signal used to
obtain the \gls{tof}~\cite{security-tof-ranging}.
However, there is no literature about 802.11az mmWave positioning, secure ranging, or its potential accuracy.



%%%%%%%%%%%%%%%%%%%%%%%
%% FTM frames FIGURE %%
%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{%
    img/FTM-frame-and-edmg-top-down-simple}
    \caption{\gls{ftm} frames (top) are Action
    fields encapsulated in the
    MAC Frame Body inside \gls{edmg} \gls{ppdu}s
    (bottom left).
    The \gls{trn} field contains Golay sequences
    (bottom right)
    used for Channel Measurements included
    in the \gls{ftm} frame.
    The figure shows
    \gls{ftm} legacy  fields (blue), so as 
    802.11az additions
    (red) and modifications (purple).
    Numbers below the \gls{ftm} frame
    indicate the
    number of octets that each field occupy.
    %{\color{red}TODO: put the Category and Public Action
    %fields fixed}
    }
    \label{fig:ftm-frames}
\end{figure*}



\bigskip

% What we do
This article contributes to the \gls{soa}
with detailed explanations of the following
procedures in 802.11az mmWave:
($i$) positioning exchanges;
($ii$) beamforming \& \gls{los} assessments; and
($iii$) secure ranging.
Additionally, we ($iv$) assess the
accuracy of 802.11az implementation using
off-the-shelf 802.11ad mmWave devices and a
\gls{soa}
solution~\cite{alejandro}.
Our experimental findings show that
802.11az mmWave implementations will achieve
errors of less than 15~cm with distances
of up to 8~m.

% How is the paper structured
The remainder of this article is organized
as follows. Sec.~\ref{sec:ftm} explains
the exchange of positioning measurements in
802.11az mmWave.
Then, Sec.~\ref{sec:fpbtlos} details
the 802.11az beamforming procedure \&
\gls{los} assessment; and
Sec.~\ref{sec:secure} explains
secure positioning with mmWave.
Finally, Sec.~\ref{sec:experimental}
shows the accuracy of future 802.11az
mmWave implementations.
Motivated by the experimental findings,
Sec.~\ref{sec:challenges} discusses
implementation challenges for 802.11az
mmWave positioning.











%%% {\color{blue}
%%% The device distance is obtained using
%%% the signal~\gls{tof}, and increasing
%%% channel bandwidths result in higher accuracy.
%%% Namely, legacy 802.11, Bluetooth and \gls{uwb}
%%% technologies~\cite{uwb-denoising,hybrid-localization}
%%% achieve decimeter-level accuracy using
%%% sub-6~GHz channels.
%%% While mmWave technologies with 60~GHz channels
%%% achieve centimeter-level accuracy.
%%% }
%%% 
%%% While the current sub-6~GHz WLANs can achieve a positioning accuracy of tens of meters to tens of centimeters~\cite{m1}, the 60~GHz WLAN with its high temporal resolution from the multi-GHz bandwidth can achieve this ultra-precise positioning accuracy. 
%%% 
%%% 
%%% In the realization of this cm-level accuracy, the next-generation WLANs in the 60~GHz band face three main challenges. First, they need to support an estimation of the distance, azimuth, and elevation between two Wi-Fi devices, which is needed for positioning (see Fig~\ref{fig:relative-positioning}). Second, knowing that the positioning performance in mmWave networks degrades when the connectivity between the two Wi-Fi devices is not directional~\cite{alejandro}, a \gls{los} assessment support is needed. Third, in order to preserve user privacy, the position estimations need to be exchanged between the Wi-Fi devices securely. 
%%% 
%%% The IEEE 802.11az amendment~\cite{802.11az} addresses these challenges, bringing new physical (PHY) and media access control (MAC) layer improvements to enable secure and accurate positioning for operation in the 60~GHz band. These new improvements include high-precision angle and \gls{tof} estimations that are exchanged between \gls{sta}s using the Fine Timing Measurement (FTM) procedure~\cite{802.11mc}. \gls{sta}s use the exchanged estimations to determine the distance, azimuth, and elevation between \gls{sta}s -- see~Fig.~\ref{fig:relative-positioning}. Furthermore, to prevent malicious \gls{sta}s to derive users’ position from the insecure \gls{ftm} exchange, 802.11az proposes a \gls{pasn} procedure to encrypt the \gls{ftm} sessions.  
%%% 
%%% \bigskip
%%% 
%%% In recent years, various works have analyzed the security~\cite{m2,security-tof-ranging}; performance and scalability~\cite{m3} features of 802.11az for operations in the sub-6~GHz band~\cite{az-sub6-finger}. However, non of the existing works in the literature discusses the  802.11az improvements for operation in the 60~GHz band that promises position accuracy with 10 times bigger resolution~\cite{m5}. This article overviews those new improvements and describes the potential benefits and challenges of each one. We have grouped these improvements into three categories: \gls{ftm} protocol over \gls{edmg},~\gls{los} assessment over the first path, and secure next-generation positioning. Moreover, we also perform an experimental analysis that shows the potential positioning accuracy of future \gls{mmwave}-based implementation of 802.11az. This is followed by a discussion of several key system-level challenges for the realization of the next-generation WLAN positioning systems 
%%% 
%%% 
%%% % SoA categories
%%% {\color{red}
%%% \begin{itemize}
%%%     \item CSI+mmWave: \cite{alejandro,passive-mmwave,mm-track}
%%%     \item security: \cite{m2,security-tof-ranging}
%%%     \item 802.11az: \cite{m3} studies the latency/positioning
%%%         tradeoff using az with communication 20~MHz and
%%%         multi-user positioning (no angle info.).
%%%         \cite{az-sub6-finger} uses 5~GHz SISO with 
%%%         channel impulse response (CIR) and AI/ML fingerprinting
%%%         (no angle information).
%%%     \item angles+TOF~\cite{mdtrack}
%%%     \item Bluetooth, UWB and multiple
%%%         technologies like WiFi for hybrid
%%%         localization~\cite{hybrid-localization}.
%%%         \cite{uwb-denoising}~to have LOS/NLOS
%%%         detection using denoising of CIR
%%%         and classification
%%% \end{itemize}
%%% }
%%% 
%%% 
%%% \todo[inline]{Jorge: why not Bluetooth, AWB
%%% or RFID. Use the 15 refs to go on 802.11az
%%% literature.}
%%% 
%%% \todo[inline]{Jorge: Mention other things that
%%% az introduces, although we do not cover it.
%%% Try to leave cristal clear that it's not a
%%% tutorial.}
%%% 
%%% \todo[inline]{Milan: for the first challenge,
%%% what is required is to \emph{exchange} angle,
%%% distance info. inside the protocol exchange
%%% (FTM).} 
%%% 
%%% \todo[inline]{Jorge/Milan: try to mention
%%% existing location techniques: fingerprinting,
%%% CSI estimations, AI/ML (cite Xavi's work).
%%% Use ANOTHER ref for AZ}
%%% 
%%% 
%%% \todo[inline]{Reviewer 1: The structure of the introduction is quite poor, and lacks several important aspects such as a description of (i) the contributions of the paper; (ii) the adopted methodology; (iii) the outcomes and results of the paper; (iv) the related works, and how (and whether) the paper overcomes literature’s limitations.}
%%% 
%%% \todo[inline]{Reviewer 1: Highly important aspects such as multi-user positioning, secure preamble (LTF), and passive positioning should be highlighted.}
%%% 
%%% 
%%% 
%%% %\gls{mmwave} WLAN positioning differs significantly from other existing positioning technologies such as visible light positioning (VLP), radio frequency identification (RFID), Bluetooth, and ultrawide-bands (UWB). In particular, WLAN positioning can provide a better transmission range while reusing the existing Wi-Fi devices which leads to a significant decrease in deployment complexity and cost.  
%%% 
%%% %https://ieeexplore.ieee.org/abstract/document/9569340 - ranging and location attacks
%%% %Multi-User Position Estimation and PerformanceTrade-offs in IEEE 802.11az WLANs
%%% %https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8436404 - IoT that mentoines az
%%% %https://www.mdpi.com/2079-9292/9/8/1193
%%% 
%%% %In particular, visible light positioning (VLP) relies on detecting the visible lights emitted by LED transmitters at known locations to determine the positions of light sensors. While implementation of VLP requires specialized equipment like photodetectors and imaging sensors, which can increase the overall cost of the system [REF], the \gls{mmwave} positioning can reuse existing Wi-Fi devices that are originally deployed for communication.  
%%% 
%%% %This amendment also offers enhancements for wireless medium utilization, power consumption, and scalable dense deployments that are not in the scope of this article. This article overviews the positioning and security features related to the mmWave WLANs that have the potential to achieve the ultra-precise positioning required by the diverse services and applications that will emerge [REF]
%%% 
%%% %In addition to the 60 GHz communication, the IEEE 802.11az amendment offers positioning enhancements for the sub-6 GHz bands. However, this lower bands can no 
%%% 
%%% 
%%% %To address those challenges, the IEEE 802.11az Task Group (802.11az for short) worked from 2015 to 2022 on an amendment~\cite{802.11az} that defines PHY and MAC layer enhancements to improve the WLAN positioning. Among other enhancements  
%%% 
%%% %The IEEE 802.11az amendment~\cite{802.11az} addresses these challenges, 
%%% 
%%% %To meet these demands, 
%%% 
%%% %az Task Group (802.11az for short) worked since 2015 to 2022 on an amendment~\cite{802.11az} that defines PHY and MAC updates for Next Generation Positioning.
%%% 
%%% 
%%% 
%%% %-how az addresses this challenges enumerate az new features, state that there are other enahncments for bla bla i bla but we foucs on the improved positioning accuracy
%%% %Among other features, that to address the cm-level positioning needs the IEEE 802.11 az amadmand proposed modificaitons ant PHY and MAC layer for mmWave ... This is the scope of our paper, however the az amadmant also offers alternatives in sub6 GHz with multi user localization but this alternative can not achive the cm-level acuracy. 
%%% 
%%% %related work and what is currently missing
%%% %Bluetooth and other alternatives for SoA and why not them... and also write the little soa that existn on az and basiclly that id does not cover the Indoor postioning in mmwave. What is the gap that we fill in in the literacure
%%% 
%%% %the contribution of this paper are:
%%% 
%%% %Although 802.11az provides enhancements for sub-6~GHz and \gls{mmwave} operation at 60~GHz, the best positioning accuracy is achieved in the latter band. Specifically, 802.11az obtains accurate positioning information using 802.11ay \gls{edmg} beamforming \cite{802.11ay}, along with its accurate \gls{csi} reports. With the orientation of the \gls{mmwave} beam and \gls{csi} reports, 802.11az elaborates angle estimations funded on the ranging accuracy of \mbox{multi-GHz} bandwidths.   
%%% 
%%% 
%%% %Unlike \gls{rssi} based solutions~\cite{localization-survey}, 802.11az combines \gls{mmwave}-based angle estimations with  the \gls{tof} to achieve high accuracy positioning. Both the \gls{tof} and angle estimations are exchanged using the \gls{ftm} procedure -- introduced in 802.11mc~\cite{802.11mc} --, and \gls{sta}s use the exchanged estimations to determine the distance, azimuth and elevation between \gls{sta}s -- see~Fig.~\ref{fig:relative-positioning}.
%%% 
%%% %Since \gls{mmwave} promises to increase positioning accuracy from meter level~\cite{MultipathTD} to centimeter-level~\cite{mmwave-survey,joan}; in this article we explain the main contributions of 802.11az for \gls{mmwave} based positioning:
%%% 
%%% 
%%% 
%%% %\textbf{FTM procedure over EDMG.} In the legacy \gls{ftm} procedure \gls{sta}s only exchange \gls{tof} estimations, thus, obtaining just an approximation of the distance. 802.11az performs the \gls{ftm} procedure over \gls{edmg} to also exchange angle estimations obtained through \gls{csi} reports. Namely, \gls{sta}s exchange  the angle at which the signals depart and arrive to the \gls{sta}, i.e., the \gls{aod} and \gls{aoa}. With the distance and angle estimations it is possible to obtain the exact position of a \gls{sta} -- see Fig.~\ref{fig:relative-positioning}.\footnote{Note that throughout the paper we use blue color for legacy features, purple color for legacy features that were extended in the IEEE 802.11az amendment and red color for new features.}
%%% 
%%% % Beamforming, FPBT & LOS assessment
%%% %\textbf{LOS assessment over the first path.} When \gls{sta}s are not at \gls{los} it becomes challenging to obtain the position due to signal reflections, e.g., on walls. Thus, it is important to determine if \gls{sta}s are at \gls{los} to derive accurate position estimations. 802.11az introduces a \gls{los} assessment procedure that tells if \gls{sta}s are at \gls{los} using dual polarization over first path transmissions. In case the \gls{los} assessment succeeds it is possible to obtain the exact position of a \gls{sta} as depicted in Fig.~\ref{fig:relative-positioning}. Otherwise, signal reflections should be considered.
%%% 
%%% % Security
%%% %\textbf{Secure Next Generation Positioning.} Since \gls{ftm} exchanges may be triggered without association, malicious \gls{sta}s may derive users' position. To prevent that, 802.11az proposes a \gls{pasn} to exchange a key used to secure \gls{ftm} sessions between not associated \gls{sta}s. Moreover, 802.11az increases the location privacy with physical security randomizing the \gls{trn} subfields used in \gls{edmg} \gls{ppdu}s. Hence, no third party can derive estimations about other \gls{sta}s location.
%%% 
%%% %\bigskip
%%% %The remainder of this article is as follows. Sec.~\ref{sec:ftm}-\ref{sec:secure} detail the main contributions of 802.11az \gls{mmwave}-based positioning. Next, Sec.~\ref{sec:experimental} assesses the accuracy of future 802.11az \gls{mmwave}-based implementations. Finally, Sec.~\ref{sec:challenges} identifies the existing challenges to be addressed while implementing \gls{mmwave}-based 802.11az.
%%% 
%%% %
%%% %-SOA background
%%% %-State clearly why no sub6
%%% %-enumerate az new features
%%% %Structure
%%% %(i) the contributions of the paper; 
%%% %(ii) the adopted methodology; 
%%% %(iii) the outcomes and results of the paper;
%%% %(iv) the related works how (and whether) the paper overcomes literature’s limitations.
%%% 
%%% 
%%% %---DO NOT INTRODUCE DIFFICULT CONCEPTS HERE, DO NOT MENTION THEM, DO NOT SUMMARY THE PAPER, USE THE INTRODUCTION STRUCTURE UP---
%%% 
%%% %refer fig1 once 1st time elev azi
%%% 
%%% %https://www.wi-fi.org/beacon/the-beacon/wi-fi-certified-location-capabilities-demonstrated-at-lisbon-member-event
%%% %this page antonio shared it, just to say there is work in progress on real implementations


==> 05_OLDexperimental.tex <==
D\section{Experimental analysis}
\label{sec:experimental}

In this section, we evaluate the positioning
accuracy using \gls{rtt} and \gls{i2r}~\gls{aoa}
estimations -- i.e. first scenario
in 802.11az~\cite[Table~11-11a]{802.11az}.
For yet there is no implementation
of \gls{mmwave} 802.11az, we resort to
legacy \gls{mmwave} \gls{ap}s to assess
the performance of future 802.11az devices.


%% Given the recent release of the 802.11az
%% amendment, there are not commercial
%% implementations of \gls{mmwave} 802.11az
%% \gls{sta}s.
%% %Since there exist no \gls{mmwave} 802.11az commercial implementation, this section evaluates the potential position accuracy of future implementations.
%% %For the experimental analysis,
%% Thus we assess the performance of future
%% commercial devices mimicking 
%% the 802.11az \gls{mmwave} features with
%% existing real-world devices.

In our experimental analysis, we use
MikroTik AP 60G, commercial-off-the-shelf hardware devices with legacy 802.11mc~\gls{ftm} support and
a \gls{mmwave} antenna array of 36 elements  with 2.16~GHz channel bandwidth.
To obtain the \gls{rtt} and \gls{i2r} \gls{aoa}
estimations of 802.11az we apply:
($i$) legacy \gls{ftm} \gls{rtt}
estimations;
and ($ii$) mD-Track~\cite{mdtrack}
\gls{i2r} \gls{aoa}
estimations using a custom version of OpenWrt -- see~\cite{alejandro}.
% Note that \gls{aoa} estimations are
% not exchanged in legacy \gls{ftm}.
%angle estimations are not exchanged in this \gls{ftm}, we obtain those estimations with a customized version of OpenWrt available in~\cite{alejandro}.
To mimic the 802.11az \gls{fpbt}
procedure we calibrate the
\gls{sta} antennas to be with 0º elevation
and the azimuths reported in
Fig.~\ref{fig:results}~(top).
%In the experimental analysis, we assume that \gls{ista} and \gls{rsta} have performed \gls{fpbt} prior to the \gls{ftm} exchange. However, since commercial devices have not yet implemented the 802.11az \gls{fpbt}, we manually orientate the \gls{sta}s to emulate the procedure.

%scenario 
The experimental scenario consists of
an \gls{ista} and six \gls{rsta}s arranged
in the room illustrated in
Fig.~\ref{fig:results}~(top).
Three \gls{rsta}s are at \gls{los}
and three at \gls{nlos}.
The three \gls{rsta}s with \gls{los} are placed 2, 4, and 8~m away from the \gls{ista};
and the signals of \gls{nlos} \gls{rsta}s 
travel 2, 4 and 8~m to reach the \gls{ista}.
%wave travel distance to make a fair comparison with the \gls{los} \gls{sta}s.
All the \gls{sta}s are placed 1~m above the floor, thus the beam's elevation is 0º.
%The beam azimuth corresponding to the
%manual orientation is illustrated in
%Fig.~\ref{fig:results}~(top~right).
%For each \gls{sta}, the selected beam's azimuth is indicated on the left side of the scenario's schematic. 

%Once the \gls{sta}s are adequately oriented,

We issue 100 legacy \gls{ftm} sessions to obtain \gls{rtt} estimations and 30
mD-Track executions for
\gls{i2r} \gls{aoa} estimations to get the distribution and minimum and maximum errors.

However, since FTM and CSI are not always carried over the same path as they are independent executions and the channel can vary, we consider all the possible matches of the 100 FTM estimations with the possible angles, considering the minimum and maximum angles experienced, for each STA.

Afterwards, we use basic trigonometry to
compute the relative position using:
($i$) \gls{ftm} \gls{rtt} estimations;
($ii$) mD-Track \gls{i2r} \gls{aoa} estimations; and
($iii$) the room shape.
%aqui igual mencionar la figura de como va el positioning

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{img/figurecommag7.pdf}
    \caption{Experiment scenario with
        \gls{los}/\gls{nlos} \gls{rsta}s
        at different distances (top).
        Results show the distance error
        CDF (bottom~left), and the
        \gls{i2r} Azimuth \& Elevation
        errors for each \gls{rsta}
    (bottom~right).}
    \label{fig:results}
\end{figure}

Figure xxx shows six curves, each corresponding to an STA. They show the variation on the position error 
%Fig.~\ref{fig:results}~(bottom~left) illustrates the distance error \gls{cdf} for the \gls{los} \gls{rsta}s (solid) and \gls{nlos} \gls{rsta}s (dashed). Results evidence that the position error increases with the distance between \gls{rsta}s, always preserving an error below 10 and
%15~cm for \gls{los} and \gls{nlos} \gls{rsta}s
%respectively. For \gls{nlos}, the measurements have higher errors and longer tails due to diffuse reflections on the walls.
%Indeed, the error for the 8~m \gls{nlos}
%\gls{rsta} shoots up to 15~cm.
%\todo[inline]{Jorge: be sure gnuplot includes the 15m xtick}

%In the case of \gls{nlos}, the error is also conditioned by the material of the wall, as it increases with rough surfaces due to diffuse reflections. As a result, to make a fair comparison, these experiments consider the same brick wall material. This phenomenon is visible as the tails of the cdf in \gls{nlos} are bigger, indicating higher variance on the distances.

%\todo[inline]{Jorge: change the order. First
%explain that the error is higher and the tails
%larger. Then you explain why. It is better
%to get the reader attention pointing directly
%to the result to capture her/his focus, and
%then you detail (the WoW effect).}
%\todo[inline]{Jorge: avoid pronouns (This).
%The pronoun here is understood as if it
%referred to the wall material, while it
%refers to the pre-prior sentence (very hard
%to follow).
%Try to avoid the sentence and resume the
%paragraph: (1) NLOS has high error and longer
%tails; and (2) you say it is because of the
%diffuse reflections of walls. Do not even
%mention they're same material.}

%Fig.~\ref{fig:results}~(bottom~right) shows the 
%\gls{i2r} \gls{aoa} azimuth (filled)
%%and elevation (empty) errors for each
%\gls{rsta}. 
%\todo[inline]{Jorge: refer to (bottom~right)
%rather than (bottom right). Be consistent.}
%\todo[inline]{Jorge: again, avoid pronouns.
%Moreover, here the use of the pronoun is not
%correct. The sentence reads as if the ``It''
%refers to the estimation errors noun, rather
%than the Fig.~6 noun. Put the two sentences into
%one and use (filled) and (dashed). Actually,
%it is hard to tell which is dashed. Rethink
%the fig.}
%For the \gls{los} \gls{rsta}s the error is between 3-4~º for both azimuth and elevation,
%being slightly higher in the azimuth because
%of calibration errors.
%\todo[inline]{Jorge: I have never read stays
%around, sounds to me like spanglish translation
%to ``se queda entorno a''. Rather, use
%``the error is between 3 and 4º''. Ah, omit
%saying the elevation innacuracy is slightly
%%higher in this sentence. Rather, mention it in
%the next one and explain why to ease the
%reading flow. Try it and see ;) }
%Since the azimuth is harder to orientate properly than the elevation (as said before, \gls{sta}s are manually oriented), the error is higher in azimuth estimations and the elevation remains close to 0º for all \gls{sta}s.
%\todo[inline]{Jorge: again the pronoun :P
%Moreover you say in the prior sentence that the
%%elevation accuracy is worse, and then you
%say that **this** is because the azimuth
%is harder to orientate. No sense.}
%\todo[inline]{Jorge: update the sentence
%to simply say ``the azimuth error is higher
%due to manual orientation errors'' -- short
%and easy. :)}
%For the \gls{nlos} \gls{sta}s, the error is higher but remains below 9~º for both azimuth and elevation. This is mainly due to irregularities in the reflections and the multipath effect, that deviates the wave from the intended trajectory.  In addition, the \gls{sta}s are more difficult to orientate, increasing the human error during this procedure.To compute the position of the \gls{nlos} \gls{sta}s (out of the scope of 802.11az) we used~\cite{mdtrack} and trigonometry approaches taking into consideration the  room's shape is known.
%\gls{nlos} \gls{rsta}s evidence higher
%azimuth and elevation errors due to reflections.
%In particular \gls{nlos} \gls{rsta}s
%experience azimuth errors below 9º, and
%elevation erros below 6º.

%\bigskip



%Overall, experiments suggest
%a promising accuracy
%for 802.11az \gls{mmwave} devices.
%Future commercial implementations will
%reach centimeter level accuracy using:
%2.16~GHz bandwidths,
%\gls{rtt} estimations, and existing
%\gls{soa} algorithms
%for \gls{i2r} \gls{aoa} estimations.
%Additionally, our experiments show that
%knowing the room shape --
%e.g. of a factory floor -- leads to
%high \gls{nlos} accuracy despite the
%reflections.
%We hypothesize that higher accuracy is
%possible by combining
%\gls{i2r} and \gls{r2i} \gls{aoa} estimations,
%or other angle combinations reported
%in~\cite[Table~11-11a]{802.11az}.

%% Overall, results show that centimeter accuracy
%% is achieved thanks to the \gls{mmwave}
%% bandwidth and \gls{rtt}/\gls{aoa} estimations.
%% We hypothesize that the
%% Overall, results show that the positioning
%% error remains below 15~cm for \gls{los}
%% and \gls{nlos}.
%% 
%% We hypothesize that 802.11az
%% implementations may increase the accuracy
%% for \gls{rsta}s will exchange not only
%% the estimations 
%% in the \gls{ftm} sessions, and 
%% In conclusion, the experiments demonstrate that LOS accuracy is excellent, and even\gls{nlos} can be accurately determined if the room shape is known. The algorithm used to determine the position in \gls{nlos} goes beyond the scope of the standard, and it is challenging if the scenario is unknown.

%\todo[inline]{Jorge: I miss a concluding
%remark of the experiments. A short paragraph
%of 1-2 sentences claiming LOS accuracy is
%super and NLOS is also in case we know the
%room shape. Additionally, we should claim
%that the algorithm is out of scope of the
%standard, and the basic trigonometry suffices
%in scenarios as the considered one. If the
%scenario is different -> challenge.}

%To compute the position of the \gls{nlos} \gls{sta}s (out of the scope of 802.11az) we used mD-Track~\cite{mdtrack} and trigonometry approaches taking into consideration the room's shape is known.

%\todo[inline]{Jorge: again, avoid the pronouns
%%(second sentence). It is way easier to structure
%as follows the whole prior paragraph:
%(1) the azimuth and elevation error is higher
%for NLOS RSTAs, yet always below 9º; and
%(2) mention that it is because the reflections.
%Do not mention the manual orientation because
%that is something present at LOS \& NLOS, is not
%the explanation on why NLOS is worse.}
%todo[inline]{Jorge: we should mention that
%mdTrack is used in the former paragraph;
%actually we should say ``mdTrack'' rather than
%[REF].}

%%\todo[inline]{Jorge: we need to mention that
%the FBPT cannot be done in the implementation.
%We need to mention that SoA is
%TM(ToA)+CSI(AoA)+MdTrack, whilst 802.11az
%is FPBT+LoS-assessment+FTM(ToA+AoA)+MdTrack.
%Measure FTM+CSI+MdTrack and claim in discussion
%that FPBT+LoS-assessment should require less
%time.}

%\todo[inline]{Jorge: compare against SoA,
%i.e. MdTrack without pointing the beam
%(FPBT+LOS). Can you repeat additional
%%experiments for 4m NLOS? If doesn't improve
%we may remove 4m and add in blue the SoA}

%We assess the positioning accuracy
%in \gls{los} and \gls{nlos} scenarios.
%In the \gls{los} scenario \gls{sta}s are
%located
%to be at \gls{los}, whilst in the
%\gls{nlos}
%scenario \gls{sta}s are separated by
%a wall, thus, the signal has to reflect
%with 60º to reach the other \gls{sta}
%-- see~Fig.~\ref{fig:results}~(top).
%In both scenarios the signal has to travel
%2~m, 4~m, and 8~m;
%regardless the \gls{sta}s
%are at \gls{los} or \gls{nlos}.




==> 05_experimental1.tex <==
%\section{Experimental analysis}
%\section{Positioning Without first-path FTM}
\section{\rev{Advanced indoor positioning experimental evaluation}}
\label{sec:experimental}



%Explain what we do, why we do it and what we expect of az
%\todo[inline]{Jorge: The first
%sentence is too long
%(more than three line
%sentences should be
%avouded). 
%%Order the ideas as follows,
%and use punctuation signs
%to write the paragraph.
%%We have three ideas:
%(i) evaluate SoA positioning;
%(ii) SoA positioning uses
%I2R AOA estimations as the
%first scenario of Table11;
%(iii) we identify the
%drawbacks that 802.11az will
%solve.
\rev{In this section, we evaluate the accuracy of an implementation of mmWave @60 GHz 802.11  that exchanges \gls{tof} and \gls{aoa} estimations over different frames. As no 802.11az implementation is available, we use our implementation to bound the performance of 802.11az future solutions. In addition, we compare other advanced indoor positioning \gls{soa} alternatives, such as 3GPP, Bluetooth 5.1, or \gls{uwb} with our implementation, and elaborate conclusions.} 

%In this section we demonstrate the
%importance of 802.11az~\gls{ftm} sessions 
%over first-path. Specifically, we 
%evaluate the positioning accuracy of an
%%\gls{soa} solution~\cite{alejandro}
%without the first-path \gls{ftm} sessions.
%The comprehensive experiments help us
%to identify the main drawback of 
%\gls{soa} solutions,
%as~\cite{alejandro}
%which is the exchange of \gls{tof} and \gls{aoa}
%estimations over different paths. 
%We observe that the mismatch between both
%estimations leads to a considerable variance
%in the positioning error.


%% PREV - first paragraph
% In this section, we evaluate the position accuracy of a 
% \gls{soa} 802.11ad based solution~\cite{alejandro}. This solution uses \gls{i2r}~\gls{aoa} estimations -- i.e. first scenario in 802.11az~\cite[Table~11-11a]{802.11az}. We identify the main drawback of the solution, which carries \gls{tof} and \gls{aoa} estimations over different paths, leading to mismatches between both estimations. The implementation in~\cite{alejandro} performs \gls{aoa} estimations using \gls{csi} beamforming training (beamsweeping) and \gls{tof} estimations over \gls{ftm}.

%In this section we evaluate the positioning accuracy using \gls{tof} and \gls{i2r}~\gls{aoa} estimations -- i.e. first scenario in 802.11az~\cite[Table~11-11a]{802.11az} with a 802.11ad based \gls{soa} solution~\cite{alejandro}, examine the drawbacks, and how 802.11az can solve them. We resort to legacy \gls{mmwave} \gls{ap}s with to discuss the performance of future 802.11az devices. These legacy devices perform \gls{aoa} estimations using \gls{csi} beamforming training (beamsweeping) and only carries \gls{tof} estimations over \gls{ftm}.


%Hardware used, how we collect data, and that it is not exactly matched
In our experimental analysis, we use MikroTik AP 60G, commercial-off-the-shelf devices with legacy 802.11mc~\gls{ftm} support and a \gls{mmwave} \rev{uniform rectangular} antenna array of 36 elements, using 2.16~GHz channel bandwidth, as specified in 802.11az. 
To obtain the \gls{tof} and \gls{i2r} \gls{aoa} estimations we apply, respectively: ($i$) 802.11ad legacy \gls{ftm}; and ($ii$) beamsweeping using a custom version of OpenWrt and mD-Track~\cite{mdtrack} to classify the obtained paths, \rev{extracting elevation, azimuth and received power.}
We calibrate the \gls{sta} antennas to be with 0º elevation and the azimuths reported in Fig.~\ref{fig:results}~(left).

%Explain the scenario, the stas with los and nlos and the distances. Explain how we calculate the nlos scenario.
The experimental scenario consists of an \gls{ista} and six \gls{rsta}s arranged in the room illustrated in Fig.~\ref{fig:results}~(left). Three \gls{rsta}s are at \gls{los} and three at \gls{nlos}. The three \gls{rsta}s with \gls{los} are placed 2, 4, and 8~m away from the \gls{ista}; and the signals of \gls{nlos} \gls{rsta}s travel 2, 4 and 8~m to reach the \gls{ista}. All the \gls{sta}s are placed 1~m above the floor, thus the beam's elevation is 0º.
%here goes the explanation of the nlos figure



%%idk where it better fits
%Since the procedures of \gls{ftm} \gls{tof} and \gls{i2r} \gls{aoa} beamsweeping are independent, \gls{tof} is not always carried over the first path calculated by \gls{aoa} beamsweeping, as the \gls{awv} can be different for each procedure due to channel variations during the measurements. This problem will be solved with an 802.11az implementation since the \gls{ftm} will carry both \gls{tof} and \gls{aoa} estimations. %esto es pq el tc<<<tiempo que tardamos en medir ambas+ el awv no es determinista en la implementación

%Explain the results, be careful, this is not az

The \gls{ista} performs beamforming to point the \gls{rsta}s. Then, the \gls{rsta} uses trigonometry to estimate the \gls{ista} position using the \gls{i2r}~\gls{aoa} and \gls{tof}-- see~Fig.~\ref{fig:results}~(right).
%The resulting beam is used to obtain the RSTA positioning using trigonometry methods with AOA and tof estimations Fig.~\ref{fig:results}~(b).
\rev{In this implementation, \gls{ftm} sessions only carry \gls{tof}, so \gls{aoa} is obtained through additional beemsweeping, resulting in extra variance in the positioning error. However, 802.11az first-path \gls{ftm} sessions will overcome it.}
%Specifically, the beam used in 
%\gls{i2r}~\gls{aoa} estimations does not
%correspond with the beam used in
%legacy~\gls{ftm} for \gls{tof} estimations, %resulting in variance
%in the positioning error.
%In other words, non-802.11az devices experience
%variance in the positioning error
%because they do not implement the first-path 
%\gls{ftm} sessions.
%As a result, we consider that the \gls{ftm} can have several azimuths and plot the position error of each STA, considering all the possible azimuths experienced.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{img/figureexperimentalcommag8.pdf}
    \caption{\rev{Experimental scenario with trigonometry approach in \gls{nlos} (left). \gls{i2r}
    \gls{aoa} errors vs. the
    positioning error (right-1).
    Legacy \gls{ftm} does not use
    first-path and introduces positioning
    error variance (\gls{tof} mismatch). Comparison between {soa} alternatives for indoor positioning (right-2).}}
    \label{fig:results}
\end{figure*}


    %Experimental scenario (a),
    %Error calculus for NLOS STAs (b), and error due to tof
    %estimations without fist-path FTM, depending on the AoA experienced (c).}

%\todo[inline]{Jorge:
%from here on
%we should explain Fig.~5 (c).
%The structure is wrong
%(and I did it :P). The
%paragraphs should be the
%follows:
%(1) explain what is the
%x-axis, y-axis, which RSTA
%correspond to each colour.
%Explain what is each
%coloured region illustrating;
%(2) explain why LOS has
%smaller error than NLOS.
%Explain why LOS finishes
%soon in the x-axis
%(the inset);
%(3) explain why is the
%large variance in the
%regions, i.e., explain
%that tofs may go over
%different paths and refer
%to the tof mismatch
%annotation; and
%(4) explain that 802.11az
%first-path FTM sessions
%will overcome the problem,
%and explain why.
%}

% Fig.~\ref{fig:results}~(bottom) shows the results obtained. The x-axis represents the \gls{aoa} error experienced for each \gls{sta}, while the y-axis is the position error, considering the variance introduced by \gls{tof} estimations. \gls{los} \gls{sta}s curves are dark-colored and \gls{nlos} \gls{sta}s curves are light-colored. As the figure shows, \gls{los} \gls{sta}s experience less error than \gls{nlos} \gls{sta}s, mainly due to lower \gls{aoa} errors experienced, as Fig.~\ref{fig:results}~(bottom-inset) shows. The variance is also smaller for \gls{los} \gls{sta}s, and it is mainly caused by \gls{tof} mismatches with \gls{aoa}, see Fig.~\ref{fig:results}~(bottom-red arrow), since they are not carried over the same path. With 802.11az, this variance will be removed, because the \gls{aoa} estimation and the \gls{tof} will be carried over the same path, and, as a result, be more accurate on the distance between \gls{sta}s measured.

Fig.~\ref{fig:results}~(right-1) plots the
\gls{i2r} \gls{aoa} error (x-axis) versus
the positioning error (y-axis) for the six
\gls{rsta}s 
in Fig.~\ref{fig:results}~(a), each
with a different color.
Results evidence that ($i$) the smaller
the distance to the \gls{rsta}s, the smaller
the positioning and \gls{i2r} \gls{aoa}
error; and ($ii$) \gls{rsta}s at \gls{los}
experience less positioning and
\gls{i2r} \gls{aoa} error than \gls{nlos}
\gls{rsta}s due to reflections.
Fig.~\ref{fig:results}~(c) inset
evidences the latter, for the \gls{rsta} at
2m~\gls{los} has a maximum
\gls{aoa} error of 5.1º in
while the \gls{rsta} at
2m~\gls{nlos} achieves a 8.3º
\gls{aoa} error.


% Comment variance
For a fixed \gls{i2r} \gls{aoa} error, the
\gls{rsta} reports different positioning
errors -- see~Fig.~\ref{fig:results}~(right-1)
regions. \rev{Such phenomena happen because the
legacy \gls{ftm} sessions do not carry the \gls{aoa} estimations, %that are performed with an additional beamsweeping procedure, 
as previously explained.}
%is not carried over the
%first-path and multiple paths
%with different \gls{tof} reach the \gls{rsta}
%reporting the same \gls{i2r} \gls{aoa}.

%802.11az first-path \gls{ftm} sessions will overcome the positioning error variance, as will travel over the first-path used for the \gls{i2r} \gls{aoa} estimation.
%This will prevent the \gls{tof} mismatch evidenced in Fig.~\ref{fig:results}~(c) results.

\rev{To provide a comprehensive understanding of the capabilities and performance of 802.11az-based positioning, we compare it with other technologies for accurate indoor positioning. The main alternatives to 802.11az are 3GPP NR cellular networks, Bluetooth 5.1 Low Energy, and \gls{uwb}. Given the \gls{soa} results achieved by these technologies in diverse scenarios, we replicate these scenarios to conduct a performance comparison with future 802.11az implementations.
For 3GPP NR, we consider two setups, the first operates at sub6 GHz ~\cite{3gpp1} and the second at\gls{mmwave} 28GHz~\cite{3gppmmwave}. The new Bluetooth 5.1 provides \gls{aoa} and \gls{aod} estimations compared to the previous version, which only provided \gls{rssi} ~\cite{bluetooth}. Last, \gls{uwb} TDOA-based algorithms can also reach good accuracy, making use of spectrum from 3.1 GHz to 10.6 GHz with a very low duty cycle~\cite{uwb}.
 
The results, as depicted in Fig.~\ref{fig:results}~(right-2), indicate that thanks to \gls{ftm} sessions with mmWave \gls{aoa} estimations, 802.11az implementations will outperform competing technologies. This superiority is achieved thanks to the high precision of a uniform rectangular array operating at 60 GHz across a 2.16 GHz bandwidth.}

%Nonetheless, these advantages come at a computational and, in terms of battery usage, a more substantial cost compared to alternatives operating at lower frequencies or power
%1 https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9601204
%TEST 5 (6.4) and TEST 1 (7.2)

%2 https://ieeexplore.ieee.org/abstract/document/9662535
%P5 (11.2)

%3 https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9771930&tag=1
%Indoor (7)

%4 UWB https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=8964963
%Indoor/m (2) (4) and (8) they get per m so we can get the ones we have

%Fig.~\ref{fig:results}~(bottom) shows how the
%\gls{rsta}s in Fig.~\ref{fig:results}~(top-left)
%increase their position error as the
%\gls{r2i}~\gls{aoa} estimation error
%increases (x-axis). As the inset in Fig.~\ref{fig:results}~(bottom) shows, \gls{los} \gls{sta}s experience
%less \gls{aoa} error, thus, their position error is always smaller on average.
%For the same angle, \gls{tof} estimations also induce error while being carried over
%non-first-path \gls{ftm} sessions. This error variance increases with small \gls{aoa} errors, since
%the \gls{tof} can deviate and be carried over other angles, being the correct estimation crucial here.
%The variance will be removed with 802.11az, because the \gls{aoa} estimation and the \gls{ftm} will be 
%carried over the same path, and, as a result, be more accurate on the distance between \gls{sta}s measured.

%Depending on the azimuth received, for both \gls{los}~(light-colored) and \gls{nlos}~(dark-colored) \gls{sta}s, we can observe the higher the distance, the higher the variance. Since \gls{aoa} is the main error source and \gls{los} \gls{sta}s tend to experience less \gls{aoa} error, the position error will always be less on average for \gls{los} \gls{sta}s, as shown in Fig.~\ref{fig:results}~(c-zoomed).

%{\color{red} talk here why the LOS end before
%%with same distance (refer to the inset).
%Then mention 
%that the error variance
%is due \gls{tof} estimations  obtained
%over non-first-path \gls{ftm} sessions.
%%Mention that the error variance increases
%with small R2I AOA error because the tof
%estimation is crucial there. Finally, state
%that the error variance will be removed
%with 802.11az, and update the plot annotation
%to something like ``error due to tof
%estimations wo/ fist-path FTM''.
%}


%{\color{red}depending on the azimuth received, for both \gls{los} (light-colored) and \gls{nlos} (dark-colored) \gls{sta}s. We can observe that the higher the distance, the higher the error variance. Since \gls{aoa} errors is the main cause of position inaccuracy and \gls{los} \gls{sta}s tend to experience fewer \gls{aoa} errors, the position error has a lower bound for \gls{los} \gls{sta}s.}
%This mainly happens because \gls{nlos} \gls{sta}s beams have small deviations in the trajectory due to the reflection, leading to more unprecise beamforming between stas.



%Discuss az adress this problems and that angle is the main source of error.
%%--PARTIALLY solved in az cause ftm will have angle and tof same frame
%%--THE MORE TRN FIELDS CONSIDER, THE BETTER ANGLE ESTIMATED, THE HIGHER ACURACCY
%%--ANGLES ARE THE MAIN CAUSE OF ERROR INTRODUCTION


==> 06_challenges.tex <==
%Collisons -> retransmisions
%How to obtain the info for the channel in real implementaion
%How does it behave on a moving object.
%Although \gls{mmwave} is envisioned as
%the main technology to achieve high
%accuracy in \gls{ngp}, it is challenging
%to distinguish between \gls{los} and
%\gls{nlos} paths. To mitigate such problem,
%recent works propose using omnidirectional 
%Sub-6~GHz antennas in cooperation with
%\gls{mmwave}~\cite{alejandro}.

%In spite of these powerful results, there are some difficulties when this technology is applied to real scenarios.
%1 ticking of the devices can derive bad measurements. This frequency is this error
%2 Moving users can cause errors because of doppler or because the estimation is not valid (user moved)
%3 battery issues: ticking freq , high freq mmwave = high battery, computation of algorithms and always listening (solved with trigger)
%if use pseudorandom codes for the TRN instead of golays it decrease quality of measurement.

%The experimental analysis from the
%prior Section evidence promising positioning
%precision in upcoming 802.11az implementations.
During the experiments
we have identified
several challenges that vendors
will have to tackle implementing
802.11az \gls{mmwave} positioning:
%However, 
% During the experimental
% analysis we have identified some challenges
% that vendors will have to tackle when
% implementing 802.11az with \gls{mmwave}:

%\todo[inline]{Jorge: it's not only through
%experimental analysis, but also after reading
%the standard and thinking.}


%\todo[inline]{Reviewer1: For instance, hardware delays, antenna calibration errors, phase noise, IQ imbalance, etc. can lead to position errors on the order of centimeters. In other words, the centimeter level accuracy is hampered by such impairments in the real-world.}

\begin{enumerate}[label=(\roman*)]

\item \textbf{Mitigate the multipath effect}. When devices are at \gls{nlos} the positioning error increases due to the presence of multipath components~\cite{multipath}, antenna calibration errors, and IQ imbalance in reflections. 
%Vendors could consider additional solutions~\cite{alejandro} that also use the sub-6~GHz channel to mitigate the multipath problem. 
  % Although 802.11az mitigates the
        %problem using \gls{scofdm} and
       % Golay sequences,
        %multipath components will remain.
        %to ensure the robustness of the transmission.
\item \textbf{Minimize energy consumption and reduce overheating}. 802.11az devices using \gls{mmwave} are highly demanding in terms of energy consumption. Energy efficient chipsets will have to avoid draining the device battery and reduce overheating upon \gls{mmwave} usage. 
        % In addition,
        % this leads to overheating, which reduces 
        % the device's performance, making them not
        % usable after 50 minutes.
  %\todo[inline]{Jorge: obtain the consumed
  %      Watts rather than showing the mAh and
  %      say that a typical mobile phone would
  %      consume it in 15' for the 1sec. FTM
  %      measurements frequency. Talk about
  %      both heating and energy consumption}
\item \textbf{Improve accurate secure positioning}. Secure \gls{trn} subfields use padded pseudorandom bit sequences rather than Golay sequences, in detriment of positioning accuracy.
A possible solution would be to use Golay sequences ciphered with homeomorphisms~\cite{homeomorphism} to preserve the autocorrelation properties.
        % Vendors may overcome the limitation
        % Looking for cyphering techniques based
        % In homeomorphisms~[REF]
        % To preserve the Golay sequences
        % Autocorrelation properties.
\end{enumerate}



%%% %the main difficulties when applying this technology to practical scenarios are listed:
%%% \begin{itemize}
%%%     \item Due to unsynchronization, a frame can be received between clock samples and not processed until the next tick. As it is commented previously, a delay of 0.1 nanoseconds causes an error of 3 centimeters in the distance measurement. 
%%% 
%%%     \item The signal is more susceptible to Doppler effect when a \gls{sta} is moving due to the use of \gls{mmwave} frequencies. This turns into bigger carrier frequency shifts, which are partially solved by using SC-OFDM and Golay sequencies but still are a problem on high speed use cases, as autonomous vehicles.
%%%     
%%%     \item EDMG frequencies impose the devices to perform high frequency ticking and have powerful chipsets to run estimation algorithms. These, together with emitting at high frequencies and over-listening to the medium, result in an extremely high consumption of the battery. Although the trigger-based \gls{ftm} implementation addresses some battery issue, it suffers from precision losses. All previous problems are translated into expensive hardware.
%%% 
%%%     \item When applied secure ranging, Golay sequences of \gls{trn} subfields are substituted by pseudo-random secure sequences, so the correlation properties of the Golay sequences are lost and may cause a reduction of accuracy. We propose to introduce homeomorphic functions, which maintain the properties, for solving the problem.
%%% 
%%%     %\item EDMG frequencies impose the devices to achieve high frequency ticking and have powerful chipsets to run estimation algorithms, which also means a extremely high consumption of battery. All these problems are translated into expensive hardware.
%%%     %\item Accessibility of information: not all commercial devices expose the \gls{ftm} and \gls{csi}. Additionally, the low rate of samples and the clock differences between the \gls{cli} (where the user obtain the information from) and chipset cause outdated data.
%%%     %\item Unsynchronization between receivers, which produces random phase offsets in the \gls{csi}, hindering to sense small changes and measure the Doppler frequency shifts. % (if we do not talk about CSI, this is not necessary).
%%%   
%%%     %\item 802.11az with EDMG drawns the battery; 
%%%     %\item EDMG @GHz freqs is expensive hardware;
%%%     %\item require high frequency ticking; and
%%%     %\item need for a more powerful chipset to run estimation algorithms
%%%     \item Vendors may decide not to implement these features in their devices, so their extended use will take a time to come.
%%% \end{itemize}

